On the robustness of the emergent spatiotemporal dynamics in biophysically realistic and phenomenological whole-brain models at multiple network resolutions

The human brain is a complex dynamical system which displays a wide range of macroscopic and mesoscopic patterns of neural activity, whose mechanistic origin remains poorly understood. Whole-brain modelling allows us to explore candidate mechanisms causing the observed patterns. However, it is not fully established how the choice of model type and the networks' resolution influence the simulation results, hence, it remains unclear, to which extent conclusions drawn from these results are limited by modelling artefacts. Here, we compare the dynamics of a biophysically realistic, linear-nonlinear cascade model of whole-brain activity with a phenomenological Wilson-Cowan model using three structural connectomes based on the Schaefer parcellation scheme with 100, 200, and 500 nodes. Both neural mass models implement the same mechanistic hypotheses, which specifically address the interaction between excitation, inhibition, and a slow adaptation current, which affects the excitatory populations. We quantify the emerging dynamical states in detail and investigate how consistent results are across the different model variants. Then we apply both model types to the specific phenomenon of slow oscillations, which are a prevalent brain rhythm during deep sleep. We investigate the consistency of model predictions when exploring specific mechanistic hypotheses about the effects of both short- and long-range connections and of the antero-posterior structural connectivity gradient on key properties of these oscillations. Overall, our results demonstrate that the coarse-grained dynamics are robust to changes in both model type and network resolution. In some cases, however, model predictions do not generalize. Thus, some care must be taken when interpreting model results.

==> tables/aln_coherence_table.tex <==
\begin{tabular}{||ll|rrrrrr||}
\hline
          & Property & \multicolumn{6}{c||}{$coh(f_{max})$} \\
          & Resolution & \multicolumn{2}{l}{100} & \multicolumn{2}{l}{200} & \multicolumn{2}{l||}{500} \\
          & Distance &            short &  long & short &  long & short &  long \\
\hline
artificial & $\textbf{C}$ &       0.69 &  0.40 &  0.44 &  0.19 &  \textbf{0.29} & \textbf{0.33} \\
          & $\textbf{C}_{weak-long}$ &       0.64 &  0.26 &  0.45 &  0.16 &  0.24 &  0.24 \\
          & $\textbf{C}_{strong-long}$ &   \textbf{0.73} & \textbf{0.52} & \textbf{0.49} & \textbf{0.28} &  0.28 &  0.31 \\
empirical & $\textbf{C}$ &   \textbf{0.69} & 0.40 & \textbf{0.44} & \textbf{0.19} & \textbf{0.29} & \textbf{0.33} \\
          & $\textbf{C}_{weak-long}$ &   \textbf{0.69} & \textbf{0.41} &  0.43 & \textbf{0.19} &  0.21 &  0.22 \\
          & $\textbf{C}_{strong-long}$ &       0.68 &  0.34 &  0.35 &  0.13 &  0.14 &  0.11 \\
\hline
\end{tabular}


==> tables/aln_psd_table.tex <==
\begin{tabular}{|| ll|rrr|rrr ||}
\hline
          & {} & \multicolumn{3}{c|}{$f_{dom}$} & \multicolumn{3}{c||}{$PSD(f_{dom})$} \\
          & Resolution &                100 &  200 &  500 &                         100 &     200 &     500 \\
\hline
artificial & $\textbf{C}$ &                0.4 &  0.4 &  0.4 &                      422.57 &  233.90 &  188.83 \\
          & $\textbf{C}_{weak-long}$ &                0.4 &  0.4 &  \textbf{0.5} &                      404.39 &  296.59 &  224.61 \\
          & $\textbf{C}_{strong-long}$ &                0.4 &  0.4 &  0.4 &                      498.04 &  246.58 &  209.31 \\
empirical & $\textbf{C}$ &                0.4 &  0.4 &  0.4 &                      422.57 &  233.90 &  188.83 \\
          & $\textbf{C}_{weak-long}$ &                0.4 &  0.4 &  \textbf{0.5} &                      558.58 &  284.15 &  179.36 \\
          & $\textbf{C}_{strong-long}$ &                0.4 &  0.4 &  \textbf{0.6} &                      482.22 &  124.25 &   97.85 \\
Standard Deviation & & 0.0 & 0.0 & 0.08 & 59 & 61 & 44 \\
\hline
\end{tabular}


==> tables/aln_sigma_mu_density_table_transposed.tex <==
\begin{tabular}{||ll|ccc|ccc||}
\hline
                &   & \multicolumn{3}{c|}{$\sigma$} & \multicolumn{3}{c||}{$\mu$} \\
                & Resolution &    100 &    200 &    500 &    100 &    200 &    500 \\
\hline
Stability &   &        &        &        &        &        &        \\
\hline
multistable & no adaptation &  0.016 &  0.012 &  0.003 &  0.009 &  0.001 & -0.002 \\
                & adaptation &  0.011 &  0.003 &  0.001 &  0.006 & -0.002 &  0.001 \\
unistable & no adaptation &  0.019 &  0.016 &  0.005 & -0.019 &  0.005 &     0 \\
                & adaptation &  \textbf{0.091} &  \textbf{0.036} &  0.003 &  0.097 &      0 & -0.001 \\
fast metastable & no adaptation &  \textbf{0.061} &  \textbf{0.025} &  \textbf{0.007} & -0.007 &  0.001 &  0.001 \\
                & adaptation &  0.069 &  0.029 &   \textbf{0.01} & -0.009 &  0.002 &  0.001 \\
slow metastable & no adaptation &  0.028 &  0.009 &  0.004 & -0.026 &  0.002 & -0.001 \\
                & adaptation &  0.031 &  0.015 &  0.007 & -0.036 & -0.002 & -0.004 \\
\hline
\end{tabular}


==> tables/wc_coherence_table.tex <==
\begin{tabular}{||ll|rrrrrr||}
\hline
          & Property & \multicolumn{6}{c||}{$coh(f_{max})$} \\
          & Resolution & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{200} & \multicolumn{2}{c||}{500} \\
          & Distance &            short &  long & short &  long & short &  long \\
\hline
artificial & $\textbf{C}$ &       0.44 &  0.12 & \textbf{0.36} &  0.09 &  0.26 &  0.23 \\
          & $\textbf{C}_{weak-long}$ &       0.43 &  0.08 &  0.34 &  0.07 &  0.17 &  0.11 \\
          & $\textbf{C}_{strong-long}$ &      \textbf{0.45} & \textbf{0.15} & \textbf{0.36} & \textbf{0.10} & \textbf{0.29} & \textbf{0.27} \\
empirical & $\textbf{C}$ &   \textbf{0.44} & \textbf{0.12} & \textbf{0.36} & \textbf{0.09} & \textbf{0.26} & \textbf{0.23} \\
          & $\textbf{C}_{weak-long}$ &       0.40 &  0.11 &  0.30 &  0.07 &  0.12 &  0.07 \\
          & $\textbf{C}_{strong-long}$ &       0.43 &  0.11 &  0.12 &  0.03 &  0.09 &  0.05 \\
\hline
\end{tabular}


==> tables/wc_psd_table.tex <==
\begin{tabular}{||ll|rrr|rrr||}
\hline
          & Property & \multicolumn{3}{c|}{$f_{dom}$} & \multicolumn{3}{c||}{$PSD(f_{dom})$} \\
          & Resolution &                100 &  200 &  500 &                         100 &   200 &   500 \\
\hline
artificial & $\textbf{C}$ &                \textbf{0.4} &  0.2 &  0.1 &                        0.21 &  0.44 &  0.75 \\
          & $\textbf{C}_{weak-long}$ &                0.3 &  0.2 &  \textbf{0.2} &                        0.21 &  0.40 &  0.54 \\
          & $\textbf{C}_{strong-long}$ &                0.3 &  0.2 &  0.1 &                        0.23 &  0.46 &  0.73 \\
empirical & $\textbf{C}$ &                \textbf{0.4} &  0.2 &  0.1 &                        0.21 &  0.44 &  0.75 \\
          & $\textbf{C}_{weak-long}$ &                \textbf{0.4} &  0.2 &  \textbf{0.2} &                        0.19 &  0.34 &  0.41 \\
          & $\textbf{C}_{strong-long}$ &                0.3 &  \textbf{0.4} &  \textbf{0.3} &                        0.20 &  0.06 &  0.27 \\
Standard Deviation & & 0.05 & 0.08 & 0.08 & 0.01 & 0.15 & 0.2 \\
\hline
\end{tabular}


==> tables/wc_sigma_mu_density_table_transposed.tex <==
\begin{tabular}{||ll|ccc|ccc||}
\hline
                &   & \multicolumn{3}{c|}{$\sigma$} & \multicolumn{3}{c||}{$\mu$} \\
                & Resolution &    100 &    200 &    500 &    100 &    200 &    500 \\
\hline
Stability &   &        &        &        &        &        &        \\
\hline
multistable & no adaptation &  0.019 &  0.005 &  0.001 &   0.01 &  0.006 &      0 \\
                & adaptation &  0.021 &  \textbf{0.015} &  \textbf{0.008} & -0.015 &  0.002 &  0.001 \\
unistable & no adaptation &  \textbf{0.041} &  \textbf{0.017} &  \textbf{0.007} & -0.003 & -0.006 & -0.001 \\
                & adaptation &  0.026 &  0.009 &  0.003 &     0 &  0.001 &     0 \\
fast metastable & no adaptation &   0.03 &  0.013 &  0.004 &  0.016 &  0.002 &  0.001 \\
                & adaptation &  \textbf{0.029} &  0.013 &  0.004 &  0.017 & -0.003 & -0.001 \\
slow metastable & no adaptation &   0.03 &  0.008 &  0.004 & -0.026 &  0.005 &      0 \\
                & adaptation &  0.023 &   0.01 &  0.008 & -0.002 &  0.002 &      0 \\
\hline
\end{tabular}

